Human biases in body measurement estimation

Body measurements, including weight and height, are key indicators of health. Being able to visually assess body measurements reliably is a step towards increased awareness of overweight and obesity and is thus important for public health. Nevertheless it is currently not well understood how accurately humans can assess weight and height from images, and when and how they fail. To bridge this gap, we start from 1,682 images of persons collected from the Web, each annotated with the true weight and height, and ask crowd workers to estimate the weight and height for each image. We conduct a faceted analysis taking into account characteristics of the images as well as the crowd workers assessing the images, revealing several novel findings: (1) Even after aggregation, the crowd's accuracy is overall low. (2) We find strong evidence of contraction bias toward a reference value, such that the weight (height) of light (short) people is overestimated, whereas that of heavy (tall) people is underestimated. (3) We estimate workers' individual reference values using a Bayesian model, finding that reference values strongly correlate with workers' own height and weight, indicating that workers are better at estimating people similar to themselves. (4) The weight of tall people is underestimated more than that of short people; yet, knowing the height decreases the weight error only mildly. (5) Accuracy is higher on images of females than of males, but female and male workers are no different in terms of accuracy. (6) Crowd workers improve over time if given feedback on previous guesses. Finally, we explore various bias correction models for improving the crowd's accuracy, but find that this only leads to modest gains. Overall, this work provides important insights on biases in body measurement estimation as obesity related conditions are on the rise.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes


==> _related_UNUSED.tex <==
\section{Related work}
\label{sec:related}

Estimating body measurements and perception biases in such judgments is an active area of research spanning multiple diverse domains, including computer science, psychology, and medicine.

\xhdr{Perception biases}
Biases in self\hyp reported weight and height estimates have been studied in medicine and behavioral psychology.
When asked to judge their own weight, people tend to systematically under- or overestimate.
For instance, it has been established through lab studies that people show a progressive underestimation of overweight and obese bodies~\cite{cornelissen2016visual}, attributed to a psychological phenomenon known as contraction bias~\cite{poulton1989bias}.
According to these studies, such underestimation may compromise people's ability to recognize weight gain and undertake compensatory weight control behaviors.
Other psychological experiments in lab settings have tried to infer mental models for how people judge height and weight.
\citet{robinson2017overweight} propose visual normalization theory to explaining why people under- or overestimate certain body shapes. 
This theory is based on the notion that weight is judged relative to the body\hyp size norms prevelant in the respective society. As larger body sizes are common in the United States, participants in \citet{robinson2017overweight}'s study assessed overweight individuals as normal.
\citet{robinson2015visual} studied a similar phenomenon for young adults from the United States (high obesity prevalence), the United Kingdom, and Sweden (lower obesity prevalence) to understand cultural differences between perceptions.
They did not find any cross-cultural difference in judging overweight males.

Based on question/answers from Yahoo!\ Answers, \citet{yom2016crowdsourced} discover that men estimate their weight fairly well, whereas women do not. This could potentially be explained by visual normalization theory (see above), where, due to societal norms on body shapes of women, being slightly over the median might be considered ``overweight'' for women but not for men.

Previous experiments have also tried to infer mental models for how people judge height.
For instance, \citet{burton2013judgments} show that people judge height from face images based on certain features such as dominance
% \note[Bob]{What is ``dominance''?}
and facial maturity, head\hyp to\hyp shoulder ratio~\cite{mather2010head}, or facial adiposity~\cite{coetzee2009facial},
while body height can be estimated using tibia (leg bone) length \cite{duyar2003body}.

People also update their perceptions when shown evidence that contradicts their mental model. For instance, \citet{robinson2014he} show that people exposed to photographs of obese young males changed their visual judgments of whether an overweight young male was of healthy weight.

As a result, statistical tools have been used to correct these biases \cite{brettschneider2015development,perez2015measuring}.
These tools usually rely on simple regression techniques to correct for under- and overestimation of light and heavy users, respectively.

\textit{Our contribution}: Our work replicates findings from small scale lab studies in a much larger setting with thousands of crowd sourcing workers. 
We find similar biases in estimating height and weight, and due to our large scale, we can provide more convincing mental models.
We also show that simple linear up or down scaling does not correct the errors to a large extent.
As a result of our setting, we can measure various aspects that were not previously possible, showing systematic biases in Estimating both weight and height based on a crowd workers own weight and height.
Using such findings can help build mental models for users.


\spara{Wisdom of crowds effects}
%
Crowdsourcing has been used in the past to estimate height and weight.
Earliest efforts in this space date back over a 100 years, when~\citet{galton1907vox} tried to use wisdom of crowds to accurately estimate the weight of an ox.

For humans, crowdsourcing has been shown to be a useful tool to assess childhood predictors of adult obesity~\cite{bevelander2014crowdsourcing},
 mental health~\cite{krieke2016hownutsarethedutch}, 
 and well being~\cite{lorincz2015revolution}.
 
However, care must be taken when using the wisdom of crowds, especially when perception biases~\cite{eickhoff2018cognitive} and social influences~\cite{lorenz2011social} creep up.
%
\citet{weber2016crowdsourcing} used crowdsourcing to obtain estimates of weight from social media profile images. 
They classify images into over weight or not and show that such estimates can in fact reconstruct county level obesity statistics in the US.
%
However, since the judgment of whether a picture
is overweight is a subjective task, depending on the human annotators who judge the image, their work suffers from the biases we report in Section~\ref{sec:}. Without accounting for such biases, the labels might not be useful.
%of conflating “overweight” with “abnormal”.

%\cite{eickhoff2018cognitive} cognitive biases in crowd sourcing.

%Another issue in using the wisdom of crowds is that they are subject to social influence, i.e.
%social influence (learning effects) \cite{lorenz2011social}
%rebuttal to that \cite{farrell2011social}

\textit{Our contribution}: Our work advances the field in two ways:
1. We try to make use of the wisdom of crowds to get valuable labels of body measurements, at the same time being conscious of biases that arise from such estimates. 
Using the wealth of supplementary data we collect, we try to infer mental models of crowdsourcing workers, that could be used to understand their biases systematically.
%
2. Using these mental models, we try to devise better crowd sourcing experiments that can help in achieving better performance, making use of wisdom of crowds for the better.

	\todo[Bob]{Also, we do regression (much harder), not binary classification}





% \spara{Machine learning models for body measurement prediction}:
% %
% Machine learning models have been built to identify height, weight and BMI of a person directly from an image (such as their Facebook profile picture).
% %
% %crowdsourcing weight estimates \cite{weber2016crowdsourcing}
% %Only label overweight or not.
% %
% \citet{wen2013computational} propose estimating BMI (Body mass index)
% based on detecting key points in each face image
% and computing hand-crafted geometric facial features to
% train a regression model.
% However, their dataset comprised of frontal face
% photos with clean background. 
% \citet{kocabey2017face} generalized this approach to work for random 
% social media images.
% They also compare their performance with human annotation and show that humans only do slightly better than the machine learning models.

% %\cite{benabdelkader2008statistical}
% \citet{gunel2018face} experiment with multiple machine learning models to predict height from an image. 
% %
% They find that height estimation from a random image is possible, and that face features help a lot in predicting height.
% Their approaches estimate height with a mean average error of 5.56cm, which is similar to what we report using human estimates.
% However, since only celebrity images were considered, a random guess produces a similar error.
% %
% Taking a different route, \citet{dey2014estimating} propose estimating heights of people from photo collections. Their approach is based on the fact that relative height differences of a similar group of people in a set of images remains the same, and hence, can be used to estimate height.

% \textit{Our contribution}: Most work in this area of automatically estimating body measurements is preliminary and builds on top of recent advances in image understanding techniques. However, as we show in this paper, the task of estimating height and weight from an image is a hard task, even for humans.
% Nevertheless, our dataset can be used for training machine learning models.
% 	\todo[Bob]{Say how}

